Extractive Summarization of Related Bug-fixing Comments in Support of Bug Repair

When developers investigate a new bug report, they search for similar previously fixed bug reports and discussion threads attached to them. These discussion threads convey important information about the behavior of the bug including relevant bug-fixing comments. Oftentimes, these discussion threads become extensively lengthy due to the severity of the reported bug. This adds another layer of complexity, especially if relevant bug-fixing comments intermingle with seemingly unrelated comments. To manually detect these relevant comments among various cross-cutting discussion threads can become a daunting task when dealing with high volume of bug reports. To automate this process, our focus is to initially extract and detect comments in the context of query relevance, the use of positive language, and semantic relevance. Then, we merge these comments in the form of a summary for easy understanding. Specifically, we combine Sentiment Analysis and the TextRank Model with the baseline Vector Space Model (VSM). Preliminary findings indicate that bug-fixing comments tend to be positive and there exists a semantic relevance with comments from other cross-cutting discussion threads. The results also indicate that our combined approach improves overall ranking performance against the baseline VSM.

==> motivation.tex <==
\subsection{Motivating Example}
\label{sec:motivation}
Consider a simplified LibreOffice bug report \#34600 described at the top of Figure~\ref{fig:bug_report_unresolved} that is in \emph{unresolved status}. As observed at the grey area of Figure~\ref{fig:bug_report_unresolved}, our tool recommends related bug-fixing comments from past resolved bugs that are extracted from their lengthy discussion threads. These recommended comments fall under the common themes of bug \#34600. For example, `comment $2$' extracted from discussions of bug \#33662 provides directions on how to handle the $90$ degree alignment issue. Similarly, `comment $3$' extracted from discussions of bug \#34436 provides concrete suggestion on what condition the problem could be eliminated. While `comment $4$' extracted from discussions of bug \#34136 and `comment $2$' of bug \#32795, confirm the fix of bug \#33622. Note that by using keyword-matching heuristic for extracting comments with keywords `fix' or `fixed' would be insufficient criterion, as, there exist other insightful comments that could capture sentiment features and patterns that are more affirmative~\cite{bahrainian2015sentiment} to problem solutions. Such examples are described in the comments from bugs \#33622 and \#34436. Both comments manifest positive sentiment of the text that can be detected by using Sentiment Analysis. The semantic connection between similar related past bugs and their corresponding discussion thread comments can be detected by using TextRank.

==> related_work.tex <==
\vspace{-0.10cm}
\section{Related Work}
\label{related_work} 
Several studies focused on ranking source files relevant to a bug report repair. Kim et \emph{al}.~\cite{KimTKZ13} applied machine learning techniques to predict source files that could fix a bug. Nguyen et \emph{al}.~\cite{NguyenNANN11} presented a tool that recommended buggy source files associated with the new bug. DebugAdvisor~\cite{AshokJLRSV09} used searches to recommend a set of similar past tasks and the source files that were changed. Saha et \emph{al}.~\cite{SahaLKP13} used bug reports and source files to build a retrieval structure for reporting bugs. Lukins et \emph{al}.~\cite{LukinsKE10} applied LDA to predict the top $10$ defective files across $22$\% of all bug reports. Ye et \emph{al}.~\cite{YeBL14} used developer domain knowledge to rank source files associated to a bug. Fujiwara et \emph{al}.~\cite{Fujiwara} used the VSM to rank bug reports to a given source file. %Lotufo et \emph{al}.~\cite{LotufoMC15} investigated an unsupervised method where sentences in a bug report were ranked based on frequently discussed topics. %Liu et \emph{al}.~\cite{LiuTZ13} introduced a learning to rank method by optimizing a set of queries and ranking functions. %Ashok et \emph{al}.~\cite{AshokJLRSV09} provided a graph-based method to recommend files and functions associated with a bug. %Linkster~\cite{BachmannBRDB10} manually linked bugs to their associated bug-fix commits. 
%Poshyvanyk et \emph{al}.~\cite{PoshyvanykGMAR07} implemented a ranking method to locate bugs for Mozilla and Eclipse. 
Recently, Hindle and Onuczko~\cite{hindle2019preventing} focused on detecting duplicate reports by continuously querying bug reports.

